Quantum State Preparation Using an Exact CNOT Synthesis Formulation

Minimizing the use of CNOT gates in quantum state preparation is a crucial step in quantum compilation, as they introduce coupling constraints and more noise than single-qubit gates. Reducing the number of CNOT gates can lead to more efficient and accurate quantum computations. However, the lack of compatibility to model superposition and entanglement challenges the scalability and optimality of CNOT optimization algorithms on classical computers. In this paper, we propose an effective state preparation algorithm using an exact CNOT synthesis formulation. Our method represents a milestone as the first design automation algorithm to surpass manual design, reducing the best CNOT numbers to prepare a Dicke state by 2x. For general states with up to 20 qubits, our method reduces the CNOT number by 9% and 32% for dense and sparse states, on average, compared to the latest algorithms.

==> algorithms/optimal-mcry-decomposition.tex <==
\begin{algorithm}[t]
\caption{Exact MCR$_y$ decomposition}\label{alg:exact-mcry-decomposition}
\SetKwInOut{Input}{input}
\SetKwInOut{Output}{output}

 \DontPrintSemicolon
 \Input{The rotation table $f$ with $n$ control qubits.}
 \Output{A sequence of quantum operators to prepare the rotation table with $K$ CNOTs.}
 
$K \gets 0$ \;
$\text{solution} \gets \varnothing$ \;
\While{$\text{solution}$ is $\varnothing$} {
    \For{$\{S_k\}$ in {$\mathbb{Z}_{n}^{\otimes K}$}} {
        $M \gets $ Construct equality system ($f$, ${S_k^i}$)\;
        solution $\gets $ Solve($M$) \;
    }
    $K \gets K+1$ \;
}
\Return solution.\;
\end{algorithm}

==> figures/qsp-example.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{images/qsp-example.pdf}
    \caption{Example of searching quantum circuits to prepare state.}
    \label{fig:qsp-example}
\end{figure*}

==> figures/random_qubits.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.7\linewidth]{images/ex-qubit-20.pdf}
    \caption{\small CNOT number comparison between our method and the most recent design automation algorithm ~\cite{mozafari2022efficient} for preparing random uniform $n$-qubit states. For each $n$, we repeat the experiment for state density $m=n$, $m=n^2$, and $m=n^3$. We plot the average number of CNOTs for each $n$.}
    \label{fig:results-rand_qubits}
\end{figure}

==> figures/random_states.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=.95\linewidth]{images/rand4.pdf}
    \caption{\small CNOT number comparison for preparing general uniform $4$-qubit states. We use the most recent design automation algorithm as the baseline~\cite{mozafari2022efficient}. We repeat the experiments $100$ times for each state density $m$. $m=1$ and $m=16$ are trivial states and omitted.}
    \label{fig:results-rand4}
\end{figure*}

==> figures/srg-example.tex <==
\begin{figure}[hbtp]
    \centering

\definecolor{offwhite}{HTML}{F2EDED}
\tikzset{> = stealth}
\resizebox{0.95\linewidth}{0.95\linewidth}{%
\begin{tikzpicture}
    \node (s0text) at (-3,0) {Final quantum state};
    \node (s0) at (0,0) {$
    \begin{bmatrix}
       0 & 0 & 1 \cr
       0 & 1 & 0 \cr
       1 & 0 & 0 \cr
    \end{bmatrix}
    $};

    \node[black] (s14) at (6,0) {$
    \begin{bmatrix}
        0 & 0 &  \textcolor{red}{0} \\
        0 & 1 &  \textcolor{red}{1}  \\
        1 & 0 &  \textcolor{red}{1}  \\
    \end{bmatrix}
    $};
    \draw[dashed] (s0) -- (s14) node [midway, above, sloped] (TextNode) {$\hat{X}_{q_0}$};
    \draw[dashed] (s0) -- (s14) node [midway, below, sloped] (TextNode) {0 CNOTs};

    % Step 1 of BDD
    \node (s1-bdd) at (-3,-3) {$
    \begin{bmatrix}
        0 & 0 & \textcolor{red}{0} \\
        0 & 1 & 0 \\
        1 & 0 & 0 \\
    \end{bmatrix}
    $};

    \draw[blue] (s0) -- (s1-bdd) node [midway, above, sloped, blue] (TextNode) {(C=$\overline{q_2q_1}$)$\hat{X}_{q_0}$};
    \draw[blue] (s0) -- (s1-bdd) node [midway, below, sloped, blue] (TextNode) {4 CNOTs};

    % Step 2 of BDD
    \node (s2-bdd) at (-6,-6) {$
    \begin{bmatrix}
        0 & \textcolor{red}{0} & 0 \\
        1 & 0 & 0 \\
    \end{bmatrix}
    $};
    
    \draw[blue] (s1-bdd) -- (s2-bdd) node [midway, above, sloped, blue] (TextNode) {(C=$\overline{q_2}$)$\hat{X}_{q_1}$};
    \draw[blue] (s1-bdd) -- (s2-bdd) node [midway, below, sloped, blue] (TextNode) {2 CNOTs};

    % Step 3 of BDD
    % \node (s3-bdd) at (-9,-9) {$
    % \begin{bmatrix}
    %     0 & 0 & 0 \\
    % \end{bmatrix}
    % $};
    
    % \draw[blue] (s2-bdd) -- (s3-bdd) node [midway, above, sloped, blue] (TextNode) {RY$_{q_2}$($\theta$)};
    % \draw[blue] (s2-bdd) -- (s3-bdd) node [midway, below, sloped, blue] (TextNode) {cost = 0};

    \node (s13) at (3,-3) {$
    \begin{bmatrix}
        0 & 0 & 1 \\
        0 & \textcolor{red}{0} & 0 \\
        1 & \textcolor{red}{1} & 0 \\
    \end{bmatrix}
    $};

   \node (s20) at (0,-6) {$
    \begin{bmatrix}
        0 & \textcolor{red}{1} & 1 \\
        0 & \textcolor{red}{1} & 0 \\
        1 & 1 & 0 \\
    \end{bmatrix}
    $};
    
    \draw[blue, dashed] (s1-bdd) -- (s20) node [midway, above, sloped, blue] (TextNode) {PXP-equivalent};
    \draw[blue, dashed] (s1-bdd) -- (s20) node [midway, below, sloped, blue] (TextNode) {0 CNOTs};

   \node (s21) at (6,-6) {$
    \begin{bmatrix}
        0 & 0 & \textcolor{red}{0} \\
        1 & 1 & 0 \\
    \end{bmatrix}
    $};
    \draw (s13) -- (s21) node [midway, above, sloped] (TextNode) {(C=$\overline{q_2}$)$\hat{X}_{q_0}$};
    \draw (s13) -- (s21) node [midway, below, sloped] (TextNode) {2 CNOTs};


   \node (s31) at (3,-9) {$
    \begin{bmatrix}
        \textcolor{red}{1} & 0 & 0 \\
        1 & 1 & 0 \\
    \end{bmatrix}
    $};
    \draw (s21) -- (s31) node [midway, above, sloped] (TextNode) {(C=$\overline{q_1}$)$\hat{X}_{q_2}$};
    \draw (s21) -- (s31) node [midway, below, sloped] (TextNode) {1 CNOT};

    \node (s30) at (-3,-9) {$
    \begin{bmatrix}
        0 & 1 & \textcolor{red}{0} \\
        1 & 1 & 0 \\
    \end{bmatrix}
    $};
    
    \draw[black, dashed] (s31) -- (s30) node [midway, above, sloped] (TextNode) {PXP-equivalent};
    \draw[black, dashed] (s31) -- (s30) node [midway, below, sloped] (TextNode) {0 CNOTs};

    \node (s40) at (0,-12) {$
    \begin{bmatrix}
        \textcolor{red}{0} & 1 & 0 \\
    \end{bmatrix}
    $};

    \node (s-final) at (6,-12) {$
    \begin{bmatrix}
         0 & \textcolor{red}{0} & 0 \\
    \end{bmatrix}
    $};
    
    \draw[dashed] (s40) -- (s-final) node [midway, above, sloped] (TextNode) {PXP-equivalent};
    \draw[dashed] (s40) -- (s-final) node [midway, below, sloped] (TextNode) {0 CNOTs};

    \draw[line width=0.5mm] (s0) -- (s13) node  [midway, above, sloped] (TextNode) {(C=$\overline{q_0}$)$\hat{X}_{q_1}$};
    \draw[line width=0.5mm] (s0) -- (s13) node  [midway, below, sloped] (TextNode) {1 CNOT};
    \draw[line width=0.5mm] (s13) -- (s20) node [midway, above, sloped] (TextNode) {(C=$\overline{q_2}$)$\hat{X}_{q_1}$};
    \draw[line width=0.5mm] (s13) -- (s20) node [midway, below, sloped] (TextNode) {1 CNOT};
    \draw[line width=0.5mm] (s20) -- (s30) node [midway, above, sloped] (TextNode) {(C=$\overline{q_2}$)$\hat{Y}_{q_0}$};
    \draw[line width=0.5mm] (s20) -- (s30) node [midway, below, sloped] (TextNode) {2 CNOTs};
    \draw[line width=0.5mm] (s30) -- (s40) node [midway, above, sloped] (TextNode) {$\hat{Y}_{q_2}$};
    \draw[line width=0.5mm] (s30) -- (s40) node [midway, below, sloped] (TextNode) {0 CNOTs};

    \draw[blue, dashed] (s2-bdd) -- (s30) node [midway, above, sloped, blue] (TextNode) {PXP-equivalent};
    \draw[blue, dashed] (s2-bdd) -- (s30) node [midway, below, sloped, blue] (TextNode) {0 CNOTs};
\end{tikzpicture}
}
    \label{fig:search-example}
    \caption{\small Example of searching shortest-distance path between the three-qubit W state and the ground state. Dashed edges are the states merged by canonicalization and thus have zero CNOT cost. The blue edges are the path found by the previous work~\cite{mozafari2022efficient}. The bold black edges are the shortest-distance path found by our algorithm. We observe that we synthesize the quantum circuit using four CNOTs while the previous work uses six CNOTs.}
\end{figure}


==> tables/canonical_3.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|ccccccc}
\hline
$q_1$ & \texttt{0} & \texttt{00} & \texttt{00} & \texttt{01} & \texttt{000} & \texttt{001} & \texttt{001} \\
$q_2$ & \texttt{0} & \texttt{00} & \texttt{01} & \texttt{01} & \texttt{001} & \texttt{001} & \texttt{010} \\
$q_3$ & \texttt{0} & \texttt{01} & \texttt{01} & \texttt{01} & \texttt{010} & \texttt{010} & \texttt{011} \\
\hline
      &
% type 1
\begin{tikzpicture}[scale = 0.3]
	%draw the axes
	\draw[blue, dashed] (0,0,0) -- (3,0,0) node[anchor=north]{$q_1$};
	\draw[blue, dashed] (0,0,0) -- (0,3,0) node[anchor=west]{$q_2$};
	\draw[blue, dashed] (0,0,0) -- (0,0,4) node[anchor=west]{$q_3$};

	%draw the top and bottom of the cube
	\draw (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;
	\draw (0,0,2) -- (0,2,2) -- (2,2,2) -- (2,0,2) -- cycle;
	\draw (0,0,0) -- (0,0,2);
	\draw (0,2,0) -- (0,2,2);
	\draw (2,0,0) -- (2,0,2);
	\draw (2,2,0) -- (2,2,2);

    % \draw (0, 0, 0) node[left=0.2cm] {$\ket{000}$};
    \draw [fill=black] (0, 0, 0) circle[radius= 0.2 cm]; 
\end{tikzpicture} &
% type 2
\begin{tikzpicture}[scale = 0.3]
	%draw the axes
	\draw[blue, dashed] (0,0,0) -- (3,0,0) node[anchor=north]{$q_1$};
	\draw[blue, dashed] (0,0,0) -- (0,3,0) node[anchor=west]{$q_2$};
	\draw[blue, dashed] (0,0,0) -- (0,0,4) node[anchor=west]{$q_3$};

	%draw the top and bottom of the cube
	\draw (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;
	\draw (0,0,2) -- (0,2,2) -- (2,2,2) -- (2,0,2) -- cycle;
	\draw (0,0,0) -- (0,0,2);
	\draw (0,2,0) -- (0,2,2);
	\draw (2,0,0) -- (2,0,2);
	\draw (2,2,0) -- (2,2,2);

    % \draw (0, 0, 0) node[left=0.2cm] {$\ket{000}$};
    \draw [fill=black] (0, 0, 0) circle[radius= 0.2 cm]; 
    \draw [fill=black] (0, 0, 2) circle[radius= 0.2 cm]; 
\end{tikzpicture} &
% type 3
\begin{tikzpicture}[scale = 0.3]
	%draw the axes
	\draw[blue, dashed] (0,0,0) -- (3,0,0) node[anchor=north]{$q_1$};
	\draw[blue, dashed] (0,0,0) -- (0,3,0) node[anchor=west]{$q_2$};
	\draw[blue, dashed] (0,0,0) -- (0,0,4) node[anchor=west]{$q_3$};

	%draw the top and bottom of the cube
	\draw (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;
	\draw (0,0,2) -- (0,2,2) -- (2,2,2) -- (2,0,2) -- cycle;
	\draw (0,0,0) -- (0,0,2);
	\draw (0,2,0) -- (0,2,2);
	\draw (2,0,0) -- (2,0,2);
	\draw (2,2,0) -- (2,2,2);

    % \draw (0, 0, 0) node[left=0.2cm] {$\ket{000}$};
    \draw [fill=black] (0, 0, 0) circle[radius= 0.2 cm]; 
    \draw [fill=black] (0, 2, 2) circle[radius= 0.2 cm]; 
\end{tikzpicture} &
% type 4
\begin{tikzpicture}[scale = 0.3]
	%draw the axes
	\draw[blue, dashed] (0,0,0) -- (3,0,0) node[anchor=north]{$q_1$};
	\draw[blue, dashed] (0,0,0) -- (0,3,0) node[anchor=west]{$q_2$};
	\draw[blue, dashed] (0,0,0) -- (0,0,4) node[anchor=west]{$q_3$};

	%draw the top and bottom of the cube
	\draw (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;
	\draw (0,0,2) -- (0,2,2) -- (2,2,2) -- (2,0,2) -- cycle;
	\draw (0,0,0) -- (0,0,2);
	\draw (0,2,0) -- (0,2,2);
	\draw (2,0,0) -- (2,0,2);
	\draw (2,2,0) -- (2,2,2);

    % \draw (0, 0, 0) node[left=0.2cm] {$\ket{000}$};
    \draw [fill=black] (0, 0, 0) circle[radius= 0.2 cm]; 
    \draw [fill=black] (2, 2, 2) circle[radius= 0.2 cm]; 
\end{tikzpicture} &
% type 5
\begin{tikzpicture}[scale = 0.3]
	%draw the axes
	\draw[blue, dashed] (0,0,0) -- (3,0,0) node[anchor=north]{$q_1$};
	\draw[blue, dashed] (0,0,0) -- (0,3,0) node[anchor=west]{$q_2$};
	\draw[blue, dashed] (0,0,0) -- (0,0,4) node[anchor=west]{$q_3$};

	%draw the top and bottom of the cube
	\draw (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;
	\draw (0,0,2) -- (0,2,2) -- (2,2,2) -- (2,0,2) -- cycle;
	\draw (0,0,0) -- (0,0,2);
	\draw (0,2,0) -- (0,2,2);
	\draw (2,0,0) -- (2,0,2);
	\draw (2,2,0) -- (2,2,2);

    % \draw (0, 0, 0) node[left=0.2cm] {$\ket{000}$};
    \draw [fill=black] (0, 0, 0) circle[radius= 0.2 cm]; 
    \draw [fill=black] (0, 0, 2) circle[radius= 0.2 cm]; 
    \draw [fill=black] (0, 2, 0) circle[radius= 0.2 cm]; 
\end{tikzpicture} &
% type 6
\begin{tikzpicture}[scale = 0.3]
	%draw the axes
	\draw[blue, dashed] (0,0,0) -- (3,0,0) node[anchor=north]{$q_1$};
	\draw[blue, dashed] (0,0,0) -- (0,3,0) node[anchor=west]{$q_2$};
	\draw[blue, dashed] (0,0,0) -- (0,0,4) node[anchor=west]{$q_3$};

	%draw the top and bottom of the cube
	\draw (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;
	\draw (0,0,2) -- (0,2,2) -- (2,2,2) -- (2,0,2) -- cycle;
	\draw (0,0,0) -- (0,0,2);
	\draw (0,2,0) -- (0,2,2);
	\draw (2,0,0) -- (2,0,2);
	\draw (2,2,0) -- (2,2,2);

    % \draw (0, 0, 0) node[left=0.2cm] {$\ket{000}$};
    \draw [fill=black] (0, 0, 0) circle[radius= 0.2 cm]; 
    \draw [fill=black] (0, 0, 2) circle[radius= 0.2 cm]; 
    \draw [fill=black] (2, 2, 0) circle[radius= 0.2 cm]; 
\end{tikzpicture} &
% type 7
\begin{tikzpicture}[scale = 0.3]
	%draw the axes
	\draw[blue, dashed] (0,0,0) -- (3,0,0) node[anchor=north]{$q_1$};
	\draw[blue, dashed] (0,0,0) -- (0,3,0) node[anchor=west]{$q_2$};
	\draw[blue, dashed] (0,0,0) -- (0,0,4) node[anchor=west]{$q_3$};

	%draw the top and bottom of the cube
	\draw (0,0,0) -- (0,2,0) -- (2,2,0) -- (2,0,0) -- cycle;
	\draw (0,0,2) -- (0,2,2) -- (2,2,2) -- (2,0,2) -- cycle;
	\draw (0,0,0) -- (0,0,2);
	\draw (0,2,0) -- (0,2,2);
	\draw (2,0,0) -- (2,0,2);
	\draw (2,2,0) -- (2,2,2);

    % \draw (0, 0, 0) node[left=0.2cm] {$\ket{000}$};
    \draw [fill=black] (0, 0, 0) circle[radius= 0.2 cm]; 
    \draw [fill=black] (0, 2, 2) circle[radius= 0.2 cm]; 
    \draw [fill=black] (2, 0, 2) circle[radius= 0.2 cm]; 
\end{tikzpicture} \\
\hline
    \end{tabular}
    \caption{\small\label{tab:example-3-input}Equivalence class representatives of $3$-qubit quantized quantum states with density $m \leq 3$.}
\end{table*}



